Actor-Critic Algorithms for Constrained Multi-agent Reinforcement Learning

In cooperative stochastic games multiple agents work towards learning joint optimal actions in an unknown environment to achieve a common goal. In many real-world applications, however, constraints are often imposed on the actions that can be jointly taken by the agents. In such scenarios the agents aim to learn joint actions to achieve a common goal (minimizing a specified cost function) while meeting the given constraints (specified via certain penalty functions). In this paper, we consider the relaxation of the constrained optimization problem by constructing the Lagrangian of the cost and penalty functions. We propose a nested actor-critic solution approach to solve this relaxed problem. In this approach, an actor-critic scheme is employed to improve the policy for a given Lagrange parameter update on a faster timescale as in the classical actor-critic architecture. A meta actor-critic scheme using this faster timescale policy updates is then employed to improve the Lagrange parameters on the slower timescale. Utilizing the proposed nested actor-critic schemes, we develop three Nested Actor-Critic (N-AC) algorithms. Through experiments on constrained cooperative tasks, we show the effectiveness of the proposed algorithms.

==> remarks.tex <==
\section{Remarks on Convergence} 
We first discuss the convergence of the centralized N-AC algorithm. 
\begin{assumption}
$\pi(\textbf{a}|s) = \pi_{1}(a_{1}|s).\pi_{2}(a_{2}|s)\ldots \pi_{n}(a_{n}|s).$
\end{assumption}

\begin{assumption}
Gradient updates in the Step 12 and Step 14 of Algorithm \ref{C-AC} are un-biased. 
\end{assumption}

\begin{lemma}
$\nabla L(\theta,\lambda)$ is Lipschitz continuous in $\theta$. 
\end{lemma}
\begin{proof}
Follows from Lemma 1 of \cite{lakshmanan2012novel}.
\end{proof}
\begin{theorem}
Algorithm \ref{C-AC} converges to near-optimal policy.
\end{theorem}
\begin{proof}
For a given set of lagrange parameters $\lambda$, $g(\lambda) = inf_{\theta} L(\theta,\lambda)$ can be computed as follows (Step 12 in Algorithm \ref{C-AC}.

\begin{align}
    \theta_{\pi_{i}} = \theta_{\pi_{i}} - a(t) (r_{t} + \gamma V_{\theta_{c}}(X_{t+1}) - V_{\theta_{c}}(X_{t})) \nabla_{\theta_{\pi_{i}}} \log \pi_{i}(a_i|X_{t})).
\end{align}

This update follows by performing stochastic gradient descent update on $g(\lambda)$ and making use of Assumptions 1 and 2 \cite{foerster2017counterfactual}. 

Similarly, $\max_{\lambda} g(\lambda)$ is computed by performing stochastic gradient ascent as follows (Step 14 in Algorithm \ref{C-AC}.

\begin{align}
    \lambda_{i_{t+1}} = max(0, \lambda_{i_{t}} + b(t)(V_{\theta_{p_i}}(X_{t}) - \alpha_{i})).
\end{align}

Finally, by making use of Lemma 1 and concept of two-time scale stochastic approximation scheme \cite{borkar1997stochastic}, we can conclude that 

\begin{align}
    (\theta^{*},\lambda^{*}) = \arg \min \max L(\theta,\lambda).
\end{align}

\end{proof}

In JAL N-AC, all the agents compute optimal actions of all the agents. Therefore, the convergence to optimal policy follows from the single agent convergence. 

Independent agents do not take into the consideration, the action of other agents. Therefore, the environment is not stationary for the agents and therefore the convergence to the optimal policy is not guaranteed. 


